Multispectral Biometrics System Framework: Application to Presentation Attack Detection

In this work, we present a general framework for building a biometrics system capable of capturing multispectral data from a series of sensors synchronized with active illumination sources. The framework unifies the system design for different biometric modalities and its realization on face, finger and iris data is described in detail. To the best of our knowledge, the presented design is the first to employ such a diverse set of electromagnetic spectrum bands, ranging from visible to long-wave-infrared wavelengths, and is capable of acquiring large volumes of data in seconds. Having performed a series of data collections, we run a comprehensive analysis on the captured data using a deep-learning classifier for presentation attack detection. Our study follows a data-centric approach attempting to highlight the strengths and weaknesses of each spectral band at distinguishing live from fake samples.

==> appendices.tex <==
% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%


\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


==> per_pai_results_table.tex <==


% \begin{table*}[!htb]
%     \caption{Caption}
%     \label{tab:analytic_results}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|cc||cccccc|cccccc|cccccc|cccccc}
%          \multicolumn{3}{c||}{} & \multicolumn{24}{c}{\textbf{PAI Category and Experiment Protocol}} \\ \toprule \hline
         
%          &  Input & \multirow{2}{*}{Metric} & \multicolumn{6}{c|}{Printed Photo} & \multicolumn{6}{c|}{Plastic Mask} & \multicolumn{6}{c|}{Makeup} & \multicolumn{6}{c}{Prostheses} \\ \hhline{~~~------------------------}
%          & Data & & & \emph{3Fold} & & & \emph{Cross} & & & \emph{3Fold} & & & \emph{Cross} & & & \emph{3Fold} & & & \emph{Cross} & & & \emph{3Fold} & & & \emph{Cross} & \\ \hline \hline

%          \multirow{21}{*}{\rotatebox[origin=c]{90}{\textbf{Face}}} & \multirow{3}{*}{RGB} & \scriptsize{AUC} 
%          & & $\mathbf{1.0000}$ & 
%          & & $0.5989$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9653$ &
%          & & $\mathbf{0.9996}$ & 
%          & & $0.9529$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9683$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{1.0000}$ & 
%          & & $0.0000$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.0873$ &
%          & & $\mathbf{0.9858}$ & 
%          & & $0.0334$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.1757$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\mathbf{0.0000}$ & 
%          & & $0.8750$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.1173$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.1773$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.1422$ & \\ \cdashline{2-27}
         
%          & \multirow{3}{*}{NDT} & \scriptsize{AUC} 
%          & & $0.9974$ & 
%          & & $0.9813$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $\mathbf{0.9997}$ &
%          & & $0.9865$ & 
%          & & $0.8226$ &
%          & & $0.9930$ & 
%          & & $0.9407$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $0.9593$ & 
%          & & $0.9009$ &
%          & & $0.9931$ & 
%          & & $0.9486$ &
%          & & $0.5140$ & 
%          & & $0.0000$ &
%          & & $0.7000$ & 
%          & & $0.0000$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $0.0014$ & 
%          & & $0.0319$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.0026$ &
%          & & $0.0269$ & 
%          & & $0.5580$ &
%          & & $0.0335$ & 
%          & & $0.1658$ & \\ \cdashline{2-27}

%          & \multirow{3}{*}{NIR-Lo} & \scriptsize{AUC} 
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9898$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9725$ &
%          & & $0.9985$ & 
%          & & $0.8580$ &
%          & & $0.9997$ & 
%          & & $0.5657$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{1.0000}$ & 
%          & & $0.8649$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.3645$ &
%          & & $0.8198$ & 
%          & & $0.0390$ &
%          & & $0.9667$ & 
%          & & $0.0167$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\mathbf{0.0000}$ & 
%          & & $0.0409$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.1216$ &
%          & & $0.0072$ & 
%          & & $0.5295$ &
%          & & $0.0019$ & 
%          & & $0.9780$ & \\ \cdashline{2-27}

%          & \multirow{3}{*}{NIR-Hi} & \scriptsize{AUC} 
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9967$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9992$ &
%          & & $0.9985$ & 
%          & & $0.9654$ &
%          & & $0.9999$ & 
%          & & $0.9719$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9865$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9533$ &
%          & & $0.7614$ & 
%          & & $0.4058$ &
%          & & $0.9667$ & 
%          & & $0.5500$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\mathbf{0.0000}$ & 
%          & & $\mathbf{0.0000}$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $\mathbf{0.0018}$ &
%          & & $0.0066$ & 
%          & & $0.1676$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.1910$ & \\ \cdashline{2-27}

%          & \multirow{3}{*}{SWIR-Lo} & \scriptsize{AUC} 
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9999$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9996$ &
%          & & $0.9984$ & 
%          & & $\mathbf{0.9936}$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $\mathbf{1.0000}$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9820$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9346$ &
%          & & $0.9116$ & 
%          & & $0.4091$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $\mathbf{1.0000}$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\mathbf{0.0000}$ & 
%          & & $\mathbf{0.0000}$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.0026$ &
%          & & $0.0037$ & 
%          & & $\mathbf{0.0057}$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $\mathbf{0.0000}$ & \\ \cdashline{2-27}

%          & \multirow{3}{*}{SWIR-Mi} & \scriptsize{AUC} 
%          & & $\mathbf{1.0000}$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9994$ &
%          & & $0.9988$ & 
%          & & $0.9900$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9999$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{1.0000}$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $\mathbf{0.9813}$ &
%          & & $0.8694$ & 
%          & & $0.6429$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $\mathbf{1.0000}$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\mathbf{0.0000}$ & 
%          & & $\mathbf{0.0000}$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.0019$ &
%          & & $0.0066$ & 
%          & & $0.0249$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.0006$ & \\ \cdashline{2-27}

%          & \multirow{3}{*}{SWIR-Hi} & \scriptsize{AUC} 
%          & & $0.9999$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $\mathbf{1.0000}$ & 
%          & & $0.9935$ &
%          & & $0.9942$ & 
%          & & $0.9699$ &
%          & & $0.9999$ & 
%          & & $\mathbf{1.0000}$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $0.9921$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $0.9972$ & 
%          & & $0.8131$ &
%          & & $0.7365$ & 
%          & & $\mathbf{0.7597}$ &
%          & & $0.9667$ & 
%          & & $\mathbf{1.0000}$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\mathbf{0.0000}$ & 
%          & & $\mathbf{0.0000}$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $0.0389$ &
%          & & $0.0346$ & 
%          & & $0.2136$ &
%          & & $\mathbf{0.0000}$ & 
%          & & $\mathbf{0.0000}$ & \\ \cline{2-27}
         
%          & \multirow{3}{*}{Mean} & \scriptsize{AUC} 
%          & & $\underline{1.0000}$ & 
%          & & $0.9999$ &
%          & & $\underline{1.0000}$ & 
%          & & $\underline{1.0000}$ &
%          & & $\underline{0.9999}$ & 
%          & & $\underline{0.9958}$ &
%          & & $\underline{1.0000}$ & 
%          & & $0.9934$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\underline{1.0000}$ & 
%          & & $0.9820$ &
%          & & $\underline{1.0000}$ & 
%          & & $\underline{0.9953}$ &
%          & & $\underline{0.9727}$ & 
%          & & $0.6364$ &
%          & & $\underline{1.0000}$ & 
%          & & $0.4333$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\underline{0.0000}$ & 
%          & & $\underline{0.0000}$ &
%          & & $\underline{0.0000}$ & 
%          & & $\underline{0.0000}$ &
%          & & $\underline{0.0000}$ & 
%          & & $0.0102$ &
%          & & $\underline{0.0000}$ & 
%          & & $0.0332$ & \\ \hline \hline

         
%          \multicolumn{1}{c}{} & & & \multicolumn{4}{c|}{Ballistic Gelatin} & \multicolumn{4}{c|}{Ecoflex Flesh} & \multicolumn{4}{c|}{2Part Silicone} & \multicolumn{4}{c|}{PDMS or Glue} & \multicolumn{4}{c|}{Cond. Silicone} & \multicolumn{4}{c}{Ecoflex Yellow} \\ \cline{4-27}
%          \multicolumn{1}{c}{} & & & \multicolumn{2}{c}{\emph{3Fold}} & \multicolumn{2}{c|}{\emph{Cross}} & \multicolumn{2}{c}{\emph{3Fold}} & \multicolumn{2}{c|}{\emph{Cross}} & \multicolumn{2}{c}{\emph{3Fold}} & \multicolumn{2}{c|}{\emph{Cross}} & \multicolumn{2}{c}{\emph{3Fold}} & \multicolumn{2}{c|}{\emph{Cross}} & \multicolumn{2}{c}{\emph{3Fold}} & \multicolumn{2}{c|}{\emph{Cross}} & \multicolumn{2}{c}{\emph{3Fold}} & \multicolumn{2}{c}{\emph{Cross}} \\ \hline \hline
         
%          \multirow{21}{*}{\rotatebox[origin=c]{90}{\textbf{Finger}}} & \multirow{3}{*}{VIS} & \scriptsize{AUC} & \multicolumn{2}{c}{$0.9999$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.9847$} & \multicolumn{2}{c|}{$0.9660$} & \multicolumn{2}{c}{$0.9889$} & \multicolumn{2}{c|}{$0.9958$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.8978$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$0.9945$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.8895$} & \multicolumn{2}{c|}{$0.7704$} & \multicolumn{2}{c}{$0.8878$} & \multicolumn{2}{c|}{$0.6395$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.6765$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$0.0006$} & \multicolumn{2}{c|}{$\mathbf{0.0000}$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$\mathbf{0.0000}$} & \multicolumn{2}{c}{$0.0163$} & \multicolumn{2}{c|}{$0.2473$} & \multicolumn{2}{c}{$0.0067$} & \multicolumn{2}{c|}{$0.0132$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$0.9921$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} \\ \cdashline{2-27}
         
%          & \multirow{3}{*}{NIR-Lo} & \scriptsize{AUC} & \multicolumn{2}{c}{$0.9972$} & \multicolumn{2}{c|}{$0.9974$} & \multicolumn{2}{c}{$0.9945$} & \multicolumn{2}{c|}{$0.9996$} & \multicolumn{2}{c}{$0.9610$} & \multicolumn{2}{c|}{$0.9711$} & \multicolumn{2}{c}{$0.9971$} & \multicolumn{2}{c|}{$0.9946$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9995$} & \multicolumn{2}{c}{$0.9522$} & \multicolumn{2}{c}{$0.6878$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$0.8647$} & \multicolumn{2}{c|}{$0.7600$} & \multicolumn{2}{c}{$0.9196$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.6900$} & \multicolumn{2}{c|}{$0.7107$} & \multicolumn{2}{c}{$0.8778$} & \multicolumn{2}{c|}{$0.7093$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9853$} & \multicolumn{2}{c}{$0.3302$} & \multicolumn{2}{c}{$0.0000$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$0.0163$} & \multicolumn{2}{c|}{$0.0071$} & \multicolumn{2}{c}{$0.0063$} & \multicolumn{2}{c|}{$0.0007$} & \multicolumn{2}{c}{$0.1272$} & \multicolumn{2}{c|}{$0.1651$} & \multicolumn{2}{c}{$0.0087$} & \multicolumn{2}{c|}{$0.0321$} & \multicolumn{2}{c}{$0.0009$} & \multicolumn{2}{c|}{$0.0010$} & \multicolumn{2}{c}{$0.1231$} & \multicolumn{2}{c}{$0.7437$} \\
%          \cdashline{2-27}
         
%          & \multirow{3}{*}{NIR-Hi} & \scriptsize{AUC} & \multicolumn{2}{c}{$0.9998$} & \multicolumn{2}{c|}{$0.9993$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9996$} & \multicolumn{2}{c}{$0.9445$} & \multicolumn{2}{c|}{$0.9678$} & \multicolumn{2}{c}{$0.9984$} & \multicolumn{2}{c|}{$0.9973$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9998$} & \multicolumn{2}{c}{$0.9910$} & \multicolumn{2}{c}{$0.9383$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$0.9797$} & \multicolumn{2}{c|}{$0.9800$} & \multicolumn{2}{c}{$0.9982$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.7375$} & \multicolumn{2}{c|}{$0.7233$} & \multicolumn{2}{c}{$0.8310$} & \multicolumn{2}{c|}{$0.6512$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.7787$} & \multicolumn{2}{c}{$0.0909$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$0.0008$} & \multicolumn{2}{c|}{$0.0015$} & \multicolumn{2}{c}{$0.0005$} & \multicolumn{2}{c|}{$0.0011$} & \multicolumn{2}{c}{$0.6331$} & \multicolumn{2}{c|}{$0.2486$} & \multicolumn{2}{c}{$0.0077$} & \multicolumn{2}{c|}{$0.0116$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$0.0004$} & \multicolumn{2}{c}{$0.0181$} & \multicolumn{2}{c}{$0.3034$} \\
%          \cdashline{2-27}
         
%          & \multirow{3}{*}{BI-$3$F} & \scriptsize{AUC} & \multicolumn{2}{c}{$0.9992$} & \multicolumn{2}{c|}{$0.9962$} & \multicolumn{2}{c}{$0.9989$} & \multicolumn{2}{c|}{$0.9959$} & \multicolumn{2}{c}{$0.9726$} & \multicolumn{2}{c|}{$0.9850$} & \multicolumn{2}{c}{$0.8812$} & \multicolumn{2}{c|}{$0.8591$} & \multicolumn{2}{c}{$0.9996$} & \multicolumn{2}{c|}{$0.9969$} & \multicolumn{2}{c}{$0.9223$} & \multicolumn{2}{c}{$0.9729$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$0.9104$} & \multicolumn{2}{c|}{$0.3376$} & \multicolumn{2}{c}{$0.9029$} & \multicolumn{2}{c|}{$0.3333$} & \multicolumn{2}{c}{$0.5648$} & \multicolumn{2}{c|}{$0.1822$} & \multicolumn{2}{c}{$0.1495$} & \multicolumn{2}{c|}{$0.0223$} & \multicolumn{2}{c}{$0.9971$} & \multicolumn{2}{c|}{$0.3724$} & \multicolumn{2}{c}{$0.1140$} & \multicolumn{2}{c}{$0.0399$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$0.0034$} & \multicolumn{2}{c|}{$0.0097$} & \multicolumn{2}{c}{$0.0054$} & \multicolumn{2}{c|}{$0.0102$} & \multicolumn{2}{c}{$0.0900$} & \multicolumn{2}{c|}{$0.0492$} & \multicolumn{2}{c}{$0.9423$} & \multicolumn{2}{c|}{$0.4288$} & \multicolumn{2}{c}{$0.0009$} & \multicolumn{2}{c|}{$0.0051$} & \multicolumn{2}{c}{$0.7731$} & \multicolumn{2}{c}{$0.0591$} \\
%          \cdashline{2-27}
         
%          & \multirow{3}{*}{SWIR-Lo} & \scriptsize{AUC} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.9935$} & \multicolumn{2}{c|}{$\mathbf{0.9995}$} & \multicolumn{2}{c}{$0.9997$} & \multicolumn{2}{c|}{$0.9894$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{0.9999}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{0.9595}$} & \multicolumn{2}{c|}{$\mathbf{0.9403}$} & \multicolumn{2}{c}{$0.9532$} & \multicolumn{2}{c|}{$0.6279$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$0.0001$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$0.0001$} & \multicolumn{2}{c}{$\mathbf{0.0016}$} & \multicolumn{2}{c|}{$\mathbf{0.0026}$} & \multicolumn{2}{c}{$0.0010$} & \multicolumn{2}{c|}{$0.0641$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$\mathbf{0.0001}$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c}{$0.0001$} \\
%          \cdashline{2-27}
         
%          & \multirow{3}{*}{SWIR-Hi} & \scriptsize{AUC} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9993$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9993$} & \multicolumn{2}{c}{$\mathbf{0.9959}$} & \multicolumn{2}{c|}{$0.9967$} & \multicolumn{2}{c}{$\mathbf{0.9998}$} & \multicolumn{2}{c|}{$0.9978$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9992$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.9993$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.9964$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.9118$} & \multicolumn{2}{c|}{$0.8227$} & \multicolumn{2}{c}{$\mathbf{0.9717}$} & \multicolumn{2}{c|}{$0.7525$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$0.9735$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$0.0014$} & \multicolumn{2}{c}{$0.0004$} & \multicolumn{2}{c|}{$0.0014$} & \multicolumn{2}{c}{$0.0056$} & \multicolumn{2}{c|}{$0.0188$} & \multicolumn{2}{c}{$\mathbf{0.0009}$} & \multicolumn{2}{c|}{$0.0090$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$0.0014$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c}{$0.0014$} \\
%          \cdashline{2-27}
         
%          & \multirow{3}{*}{LSCI-$3$F} & \scriptsize{AUC} & \multicolumn{2}{c}{$0.9943$} & \multicolumn{2}{c|}{$0.9995$} & \multicolumn{2}{c}{$0.9998$} & \multicolumn{2}{c|}{$0.9999$} & \multicolumn{2}{c}{$0.9382$} & \multicolumn{2}{c|}{$0.9759$} & \multicolumn{2}{c}{$0.9995$} & \multicolumn{2}{c|}{$\mathbf{0.9998}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{0.9999}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.9999$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$0.9321$} & \multicolumn{2}{c|}{$0.9400$} & \multicolumn{2}{c}{$0.9799$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$0.7829$} & \multicolumn{2}{c|}{$0.7916$} & \multicolumn{2}{c}{$\mathbf{0.9717}$} & \multicolumn{2}{c|}{$\mathbf{0.9884}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c|}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} & \multicolumn{2}{c}{$\mathbf{1.0000}$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$0.0029$} & \multicolumn{2}{c|}{$0.0020$} & \multicolumn{2}{c}{$0.0009$} & \multicolumn{2}{c|}{$0.0002$} & \multicolumn{2}{c}{$0.7915$} & \multicolumn{2}{c|}{$0.1557$} & \multicolumn{2}{c}{$\mathbf{0.0009}$} & \multicolumn{2}{c|}{$\mathbf{0.0008}$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c|}{$0.0002$} & \multicolumn{2}{c}{$\mathbf{0.0000}$} & \multicolumn{2}{c}{$0.0005$} \\ \cline{2-27}
         
%           & \multirow{3}{*}{Mean} & \scriptsize{AUC} & \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c|}{$\underline{1.0000}$} & \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c|}{$\underline{1.0000}$} & \multicolumn{2}{c}{$\underline{0.9973}$} & \multicolumn{2}{c|}{$0.9988$} & \multicolumn{2}{c}{$\underline{0.9999}$} & \multicolumn{2}{c|}{$0.9986$} & \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c|}{$\underline{0.9999}$} & \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c}{$0.9988$} \\
%          & & \scriptsize{TPR$0.2\%$} & 
%          \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c|}{$\underline{1.0000}$} & \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c|}{$\underline{1.0000}$} & \multicolumn{2}{c}{$0.9448$} & \multicolumn{2}{c|}{$0.8302$} & \multicolumn{2}{c}{$\underline{0.9810}$} & \multicolumn{2}{c|}{$0.7558$} & \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c|}{$\underline{1.0000}$} & \multicolumn{2}{c}{$\underline{1.0000}$} & \multicolumn{2}{c}{$0.8701$} \\
%          & & \scriptsize{BPCER$20$} & 
%          \multicolumn{2}{c}{$\underline{0.0000}$} & \multicolumn{2}{c|}{$\underline{0.0000}$} & \multicolumn{2}{c}{$\underline{0.0000}$} & \multicolumn{2}{c|}{$\underline{0.0000}$} & \multicolumn{2}{c}{$0.0024$} & \multicolumn{2}{c|}{$0.0084$} & \multicolumn{2}{c}{$\underline{0.0008}$} & \multicolumn{2}{c|}{$0.0051$} & \multicolumn{2}{c}{$\underline{0.0000}$} & \multicolumn{2}{c|}{$0.0002$} & \multicolumn{2}{c}{$0.0008$} & \multicolumn{2}{c}{$0.0027$} \\ \hline \hline
         
%          \multicolumn{1}{c}{} & & & \multicolumn{6}{c}{Fake Eyes} & \multicolumn{6}{c}{Air Optix CL} & \multicolumn{6}{c}{Intrigue CL} & \multicolumn{6}{c}{Special CL} \\ \cline{4-27}
%          \multicolumn{1}{c}{} & & & & \emph{3Fold} & & & \emph{Cross} & & & \emph{3Fold} & & & \emph{Cross} & & & \emph{3Fold} & & & \emph{Cross} & & & \emph{3Fold} & & & \emph{Cross} & \\ \hline \hline
         
%          \multirow{18}{*}{\rotatebox[origin=c]{90}{\textbf{Iris}}} & \multirow{3}{*}{N$780$} & \scriptsize{AUC} 
%          & & $\mathbf{0.9888}$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $0.9962$ & 
%          & & $0.9963$ &
%          & & $0.9960$ & 
%          & & $\mathbf{0.9989}$ &
%          & & $\mathbf{0.9930}$ & 
%          & & $\mathbf{0.9997}$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{0.9778}$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $0.9108$ & 
%          & & $0.9519$ &
%          & & $0.9333$ & 
%          & & $0.9286$ &
%          & & $0.6485$ & 
%          & & $\mathbf{1.0000}$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $0.0013$ & 
%          & & $\mathbf{0.0000}$ &
%          & & $0.0061$ & 
%          & & $\mathbf{0.0015}$ &
%          & & $0.0563$ & 
%          & & $0.0063$ &
%          & & $0.0350$ & 
%          & & $\mathbf{0.0015}$ & \\ \cdashline{2-27}
         
%          & \multirow{3}{*}{N$850$} & \scriptsize{AUC} 
%          & & $0.9856$ & 
%          & & $0.9958$ &
%          & & $0.9985$ & 
%          & & $0.9873$ &
%          & & $0.9812$ & 
%          & & $0.9611$ &
%          & & $0.9914$ & 
%          & & $0.9841$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $0.9556$ & 
%          & & $0.9333$ &
%          & & $0.8556$ & 
%          & & $0.6442$ &
%          & & $0.4852$ & 
%          & & $0.3214$ &
%          & & $0.6620$ & 
%          & & $0.2500$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $0.0017$ & 
%          & & $0.0633$ &
%          & & $\mathbf{0.0057}$ & 
%          & & $0.0883$ &
%          & & $0.1603$ & 
%          & & $0.2163$ &
%          & & $\mathbf{0.0298}$ & 
%          & & $0.0559$ & \\ \cdashline{2-27}
         
%          & \multirow{3}{*}{N$870$} & \scriptsize{AUC} 
%          & & $0.9834$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $\mathbf{0.9976}$ & 
%          & & $0.9903$ &
%          & & $0.9398$ & 
%          & & $0.9154$ &
%          & & $0.9912$ & 
%          & & $0.9543$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{0.9778}$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $0.7465$ & 
%          & & $0.6154$ &
%          & & $0.3873$ & 
%          & & $0.1786$ &
%          & & $0.\mathbf{6783}$ & 
%          & & $0.1875$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $0.0009$ & 
%          & & $\mathbf{0.0000}$ &
%          & & $0.0141$ & 
%          & & $0.0442$ &
%          & & $0.4822$ & 
%          & & $0.2980$ &
%          & & $0.0410$ & 
%          & & $0.2377$ & \\ \cdashline{2-27}
         
%          & \multirow{3}{*}{N$940$} & \scriptsize{AUC} 
%          & & $0.9855$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $0.9884$ & 
%          & & $0.9755$ &
%          & & $0.9028$ & 
%          & & $0.7653$ &
%          & & $0.9779$ & 
%          & & $0.9574$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $0.8481$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $0.4344$ & 
%          & & $0.3173$ &
%          & & $0.0000$ & 
%          & & $0.0000$ &
%          & & $0.2415$ & 
%          & & $0.1250$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $0.0029$ & 
%          & & $\mathbf{0.0000}$ &
%          & & $0.0318$ & 
%          & & $0.1100$ &
%          & & $0.4843$ & 
%          & & $0.4433$ &
%          & & $0.0979$ & 
%          & & $0.1582$ & \\ \cdashline{2-27}
         
%          & \multirow{3}{*}{IrisID} & \scriptsize{AUC} 
%          & & $0.9843$ & 
%          & & $0.9998$ &
%          & & $0.9923$ & 
%          & & $\mathbf{0.9969}$ &
%          & & $\mathbf{0.9979}$ & 
%          & & $0.9961$ &
%          & & $0.9821$ & 
%          & & $0.9878$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\mathbf{0.9778}$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $\mathbf{0.9266}$ & 
%          & & $\mathbf{0.9808}$ &
%          & & $\mathbf{0.9762}$ & 
%          & & $\mathbf{0.9643}$ &
%          & & $0.6333$ & 
%          & & $0.6250$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\mathbf{0.0004}$ & 
%          & & $0.0007$ &
%          & & $0.0219$ & 
%          & & $\mathbf{0.0015}$ &
%          & & $\mathbf{0.0009}$ & 
%          & & $\mathbf{0.0011}$ &
%          & & $0.0839$ & 
%          & & $0.0751$ & \\ \cdashline{2-27}
         
%          & \multirow{3}{*}{Thermal} & \scriptsize{AUC} 
%          & & $0.9880$ & 
%          & & $0.9995$ &
%          & & $0.8881$ & 
%          & & $0.9182$ &
%          & & $0.7457$ & 
%          & & $0.8484$ &
%          & & $0.8919$ & 
%          & & $0.7154$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $0.8056$ & 
%          & & $\mathbf{1.0000}$ &
%          & & $0.0048$ & 
%          & & $0.0769$ &
%          & & $0.0000$ & 
%          & & $0.0714$ &
%          & & $0.1068$ & 
%          & & $0.0000$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $0.0157$ & 
%          & & $0.0007$ &
%          & & $0.3642$ & 
%          & & $0.3013$ &
%          & & $0.8587$ & 
%          & & $0.5677$ &
%          & & $0.5239$ & 
%          & & $0.9264$ & \\ \cline{2-27}
         
%          & \multirow{3}{*}{Mean} & \scriptsize{AUC} 
%          & & $\underline{0.9965}$ & 
%          & & $\underline{1.0000}$ &
%          & & $\underline{0.9999}$ & 
%          & & $\underline{0.9998}$ &
%          & & $\underline{0.9997}$ & 
%          & & $\underline{0.9996}$ &
%          & & $0.9926$ & 
%          & & $0.9898$ & \\
%          & & \scriptsize{TPR$0.2\%$}
%          & & $\underline{0.9778}$ & 
%          & & $\underline{1.0000}$ &
%          & & $\underline{0.9706}$ & 
%          & & $0.9615$ &
%          & & $0.8889$ & 
%          & & $0.9286$ &
%          & & $\underline{0.6919}$ & 
%          & & $0.6250$ &\\
%          & & \scriptsize{BPCER$20$} 
%          & & $\underline{0.0000}$ & 
%          & & $\underline{0.0000}$ &
%          & & $\underline{0.0013}$ & 
%          & & $\underline{0.0011}$ &
%          & & $0.0026$ & 
%          & & $0.0022$ &
%          & & $0.0514$ & 
%          & & $0.0876$ & \\ \hline \bottomrule
         
%     \end{tabular}}
% \end{table*}

